Human-Aware Physical Human-Robot Collaborative Transportation and Manipulation with Multiple Aerial Robots

Human-robot interaction will play an essential role in various industries and daily tasks, enabling robots to effectively collaborate with humans and reduce their physical workload. Most of the existing approaches for physical human-robot interaction focus on collaboration between a human and a single ground or aerial robot. In recent years, very little progress has been made in this research area when considering multiple aerial robots, which offer increased versatility and mobility. This paper proposes a novel approach for physical human-robot collaborative transportation and manipulation of a cable-suspended payload with multiple aerial robots. The proposed method enables smooth and intuitive interaction between the transported objects and a human worker. In the same time, we consider distance constraints during the operations by exploiting the internal redundancy of the multi-robot transportation system. The key elements of our approach are (a) a collaborative payload external wrench estimator that does not rely on any force sensor; (b) a 6D admittance controller for human-aerial-robot collaborative transportation and manipulation; (c) a human-aware force distribution that exploits the internal system redundancy to guarantee the execution of additional tasks such inter-human-robot separation without affecting the payload trajectory tracking or quality of interaction. We validate the approach through extensive simulation and real-world experiments. These include scenarios where the robot team assists the human in transporting and manipulating a load, or where the human helps the robot team navigate the environment. We experimentally demonstrate for the first time, to the best of our knowledge, that our approach enables a quadrotor team to physically collaborate with a human in manipulating a payload in all 6 DoF in collaborative human-robot transportation and manipulation tasks.

==> sections/04-Interaction_fullUKFdescription.tex <==
\section{Human-Robot Physical Interaction}\label{sec:admittance}
\subsection{State Estimation}
In this section, we present a method of state estimation based on an Unscented Kalman Filter (UKF). The estimation design is fully distributed. We included unit cable direction and cable tension magnitude as part of the state estimation, which enables us to estimate the amount of external force applied on the payload by the human operator through eq.~(\ref{eq:total_wrench_on_payload}). State estimation is performed fully onboard each MAV. The distributed nature of our method allows the entire system to be scaled easily. Since the estimation algorithm runs onboard, the computation cost per robot does not increase as the swarm gets large. The distributed design also reduces possible interference among robots as estimation algorithms are running independently in a parallel fashion. Below, we will discuss the UKF-based MAV state estimation in Section~\ref{sec:Robot_Estimator} and how we estimate the payload external wrench in Section~\ref{sec:Wrench_Estimator}.

\subsubsection{Robot State Estimator}\label{sec:Robot_Estimator}
We consider the $\id^{th}$ MAV to have the following state $\state{\id}$
\begin{equation}
    \state{\id}=\begin{bmatrix}
    \robotpos{\id} & \robotvel{\id}  & \robotypr{\id} & \robotangvel{\id}  & \cablevec{\id} & \cabledotvec{\id} & \scalartension{\id}
    \end{bmatrix}^{\top},
\end{equation}
where $\robotypr{\id}$ are the robot orientation Euler angles expressed according to the ZYX convention and the input are defined as
\begin{equation}
    \ekfinputi = \begin{bmatrix}f_{\id}&\qdM{\id}^{\top}\end{bmatrix}^{\top},
\end{equation}
where $\acci$ is defined in the dynamic model and the $\id^{th}$ attach point and $f_{\id}$ is obtained based on motor speed values from the electronic speed controllers as
\begin{equation}
    f_{\id} = \sum_{j=1}^{4}k_f\omega_{mj}^2,\label{eq:motor_speed}
\end{equation}
where $k_f$ is the known motor constant, $\omega_{mj}$ is the motor speed of the $j^{th}$ motor. Denote the current time step as $*^t$ and the previous time step as $*^{t-1}$. Now we will present the nonlinear process model and the linear measurement model of the UKF. 
\paragraph{Process Model}
Based on MAV equations of motion presented in eq.~(\ref{eq:quad_eom_rot_dropped}), discretizations of quadrotor states are performed by assuming each control step moves forward in time by $\delta t$. The discrete-time nonlinear process model with noise on each robot is, therefore:
\begin{equation}
    \state{\id}^{t} = g(\state{\id}^{t-1}, \controlin{\id}^{t}, \processnoise{\id}^{t-1}, \delta t).
\end{equation}
where $\processnoise{\id}^{t-1}$ is the process noise as an input to the process model:
\begin{equation}
    \processnoise{\id}^{t-1}=\begin{bmatrix}
        \mathbf{n}_{f, \id}^{t-1}&
        n_{\mu, \id}^{t-1}&
        \mathbf{n}_{\cablevec{}, \id}^{t-1}&
        \mathbf{n}_{\qdM{}, \id}^{t-1}&
        \mathbf{n}_{\robotangvel{}, \id}^{t-1}&
        \mathbf{n}_{\cabledotvec{}, \id}^{t-1}
    \end{bmatrix}^{\top}
\end{equation}
The process model is:
\begin{equation}
\begin{split}
\state{\id}^{t}&=\begin{bmatrix}
    \robotpos{\id}^{t-1}+\robotvel{\id}^{t-1}\delta t+\robotacc{\id}^{t}\frac{\delta t^2}{2}\\
    \robotvel{\id}^{k-1}+\robotacc{\id}^{t}\delta t\\
    \left\lfloor\robotrot{\id}^{t-1}\textbf{exp}\left[\robotrot{\id}^{t-1}\robotangvel{\id}^{t-1}\delta t\right]\right\rfloor\\
    \robotangvel{\id}^{t-1}+\robotangacc{\id}^{t}\delta t\\
    \cablevec{\id}^{t-1}+\cabledotvec{\id}^{t}\delta t+\cableddotvec{\id}^{t}\frac{\delta t^2}{2}+\mathbf{n}_{\cablevec{}, \id}^{t-1}\\
    \cabledotvec{\id}^{t-1}+\cableddotvec{\id}^{t}\delta t+\mathbf{n}_{\cabledotvec{}, \id}^{t-1}\\
    \scalartension{\id}^{t-1}+n_{\mu, \id}
    \end{bmatrix}\\
\end{split}.
\label{eq:nonlinear_process_model}
\end{equation}
where $\robotacc{\id}^{t} = [\robotrot{\id}^{t-1}(f_{\id}^{t}+\mathbf{n}_{f, \id}^{t-1})+(\cablevec{\id}^{t-1}+\mathbf{n}_{\cablevec{}, \id}^{t-1})(\scalartension{\id}^{t-1}+n_{\mu, \id}^{t-1})]\frac{1}{\massi}-\begin{bmatrix}
    0&0&9.81
\end{bmatrix}^{\top}$ and $\robotangacc{\id}^{t} =\inertia_{\id}^{-1}[(\qdM{\id}^{t}+\mathbf{n}_{\qdM{}, \id}^{t-1})-(\robotangvel{\id}+\mathbf{n}_{\robotangvel{}, \id}^{t-1})\times\inertia_{\id} (\robotangvel{\id}+\mathbf{n}_{\robotangvel{}, \id}^{t-1})]$.
For updating the Euler angle, a few nonlinear mappings are used as in \cite{sola2017quaternion}
\begin{enumerate}
    \item $\lfloor*\rfloor$ that maps $*\in\SOthree$ to $\robotypr{}\in\realnum{3}$.
    \item $\textbf{exp}[*]$ that maps $*\in\realnum{3}$ to $\SOthree$; or maps axis-angle $\mathfrak{so}(3)$, to rotation matrix $\SOthree$. 
\end{enumerate} 
In eq.~(\ref{eq:nonlinear_process_model}), $\robotangvel{\id}^{t-1}$ is rotated into $\worldf$. After stepping $dt$, the new robot angular position in $\worldf$ represented in $\mathfrak{so}(3)$ is mapped into $\SOthree$. This new angular position in $\SOthree$ is then added to the previous orientation. The resultant orientation is mapped to the Euler angle with $\lfloor*\rfloor$. The noise terms, $\mathbf{n}_{f, \id}, \mathbf{n}_{\cablevec{}, \id}, \mathbf{n}_{\qdM{}, \id}, \mathbf{n}_{\robotangvel{}, \id},\mathbf{n}_{\cabledotvec{}, \id}\in\realnum{3}$ and $n_{\mu, \id}\in\realnum{}$, are considered within the process model. Gaussian white noise is also considered as process noise for linear and angular acceleration.
Additionally, the equations of motion for unit cable direction are presented in \cite{guanrui2021ral}. Here, we provide the result. Gaussian white noise, $\processnoise{\id}$, is added as process noise
\begin{equation}
\begin{split}
\begin{bmatrix}\cabledotveci^t\\\vspace{-8pt}\\\cableddotvec{\id}^t\end{bmatrix}= 
\begin{bmatrix}\cabledotvec{\id}^t\\
\frac{\left(\hat{\cablevec{}}^{t-1}_{\id}\right)^2\prths{\inputforce{\id}-\massi\acci}}{\massi l_{\id}}-\twonorm{\cabledotveci^{t-1}}^2\cableveci^{t-1}\end{bmatrix}\hspace{-2pt} + \begin{bmatrix}
    \mathbf{n}_{\cablevec{}, \id}^{t-1}\\
    \mathbf{n}_{\cabledotvec{}, \id}^{t-1}
\end{bmatrix}.
\end{split}
\end{equation}
To predict with the process model, the UKF algorithm calls eq.~(\ref{eq:nonlinear_process_model}). Since measurement does not necessarily arrive at every control time step, nonlinear prediction with zero process noise is used.
\paragraph{Measurement Model}
Using an indoor MOCAP system, we can measure everything in the state except tension magnitude. The measured states for $\id^{th}$ robot therefore are
\begin{equation}
    \measurement{\id}= \begin{bmatrix}
    % \robotpos{\id} & \robotvel{\id} & \robotacc{\id} & \robotypr{\id} & \robotangvel{\id} & \robotangacc{\id} & \qdF{\id} & \qdM_{\id}
    \robotpos{\id} & \robotvel{\id}  & \robotypr{\id} & \robotangvel{\id}  & \cablevec{\id} & \cabledotvec{\id}
    \end{bmatrix} ^{\top}.
\end{equation}
We also want to note that using onboard Visual Inertial Odometry and vision-based methods from our previous work \cite{guanrui2021ral} can provide the exact measurements and make measurements fully onboard. 

Denoting the time step when UKF measurement update is triggered as $m$, the UKF finds the state prior to $m$, $\state{\id}^{m-1}$. A nonlinear propagation through eq.~(\ref{eq:nonlinear_process_model}) is performed by propagating sigma points around $\state{\id}^{m-1}$ through the system model in eq.~(\ref{eq:nonlinear_process_model}) as shown in~\cite{thrun_probabilistic_robotics}. 

The linear measurement model is
$$\measurementmodel =  \begin{bmatrix}
    \mathbf{I}_{18\times18}&\mathbf{0}_{18\times1}\\
    \mathbf{0}_{1\times18}&\mathbf{0}_{1\times1}\\
\end{bmatrix}.$$
The system state prediction is compared to the actual measurement using the above model
\begin{equation}
    \state{\id}^m =\kalmangain{\id}(\measurementmodel
    \statebar{\id}^{m}-\measurement{\id}),
\end{equation}
where $\statebar{\id}^{m}$ is the averaged state after sigma point propagation and $\kalmangain{\id}$ is the Kalman gain. Kalman gain is computed based on the standard UKF update step as in \cite{thrun_probabilistic_robotics}.

\subsubsection{Payload Wrench Estimator}\label{sec:Wrench_Estimator}
Rearranging eq.~(\ref{eq:total_wrench_on_payload}), we obtain
\begin{equation}
   \begin{bmatrix}\loadmass\loadacc\\\inertiaload\loadangacc\end{bmatrix}=\begin{bmatrix}\extplF \\ \extplM\end{bmatrix}+{\matP}\begin{bmatrix}\tension{1}\\\vdots\\\tension{n}\end{bmatrix}-\begin{bmatrix}
    m\vecg\\
    \mathbf{0}_{3\times1}
    \end{bmatrix}.
    \label{eq:payload_extest}
\end{equation}
Considering quasi-static operating conditions, we can assume payload linear and angular accelerations are small. Therefore, leveraging this assumption and rearranging based on eq.~(\ref{eq:payload_extest}) we obtain
\begin{equation}
\begin{split}
   \begin{bmatrix}\extplF \\ \extplM\end{bmatrix}&=-{\matP}\begin{bmatrix}\tension{1}\\\vdots\\\tension{n}\end{bmatrix}+\begin{bmatrix}
    m\vecg\\
    \mathbf{0}_{3\times1}
    \end{bmatrix}.
\end{split}
\end{equation}
Extracting tension values from each robot's state allows us to compute the external wrenches on the payload.

\subsection{Payload Admittance Controller} \label{sec:admittance_controller}
The admittance controller is a high-level controller that updates $\loadposdes$ and $\loadrotdes$ in eq.~(\ref{eq:control_errors}) for the payload controller (Section~\ref{sec:payload_controller}) based on the external force applied on the payload. When interacting with the payload, it allows the human operator to experience a virtual mass-spring-damper system instead of the actual mass. By setting the admittance controller's tunable parameters to the desired values, the payload can be either sensitive or insensitive to external forces regardless of the payload's actual property. 

The admittance controller treats the payload as a virtual mass-spring-damper system as the external force applied to the payload. The input is a payload external wrench, $\wrench\in\realnum{6\times1}$. The output includes payload twist, $\dot{\mathcal{X}}_{des}\in\realnum{6\times1}$, and payload linear and angular position, $\mathcal{X}_{des}\in\realnum{6\times1}$, with angular position represented by Euler angle. Admittance controller also computes payload linear and angular acceleration, $\Ddot{\mathcal{X}}_{des}\in\realnum{6\times1}$, but the lower level payload controller does not use this output.
The controller assumes the following dynamics for the payload,
\begin{equation}
    \mathbf{M}(\Ddot{\mathcal{X}}_{des}-\Ddot{\mathcal{X}}_{traj})+\mathbf{D}(\dot{\mathcal{X}}_{des}-\dot{\mathcal{X}}_{traj})+\mathbf{K}(\mathcal{X}_{des}-\mathcal{X}_{traj})=\wrench,
    \label{eq:admittance_ctrl}
\end{equation}
where $\mathbf{M}$, $\mathbf{D}$, and $\mathbf{K}\in\realnum{6\times6}$ are tunable positive semidefinite matrices denoting the desired mass, damping, and spring property of the payload. Based on the initial starting condition of the payload, $\Ddot{\mathcal{X}}_{traj}$, $\dot{\mathcal{X}}_{traj}$, and $\mathcal{X}_{traj}$ can be set accordingly. We choose to set them to be the planned trajectory.
Closed-form solutions exist for eq.~(\ref{eq:admittance_ctrl}) with the assumption that $\wrench$ is a predetermined function (e.g., a linear function). However, such an assumption is not ideal for our use case. Thus, we choose to solve $\mathcal{X}_{des}$, $\dot{\mathcal{X}}_{des}$, $\Ddot{\mathcal{X}}_{des}$ with Runge-Kutta $4^{th}$ order approximation.  

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/force_sensor_module.png}
    \caption{Wrench estimation evaluation. The human operator uses a force measurement device to measure the applied wrench on the payload, which is used to validate our wrench estimation algorithm results. Force application via the force measurement device (left) and force measurement device (right).}
    \label{fig:wrench_measurement_device}
\end{figure}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/experiments/wrench_measurements.png}
    \caption{Wrench estimation experiment results. Comparison between the wrench estimation algorithm results and the wrench measurements from the force measurement device in all 6 DoF.}
    \label{fig:wrench_measurement}
\end{figure*}



==> sections/archived.tex <==
%\begingroup
%\endgroup
%Let $\worldf$ be the inertial frame, or the world frame, with axes $\{\axis{x}{},\axis{y}{},\axis{z}{}\}$. The frame of the $i$th robot is denoted as $\robotframe{i}$ with axes $\{\axis{x}{\robotframe{i}},\axis{y}{\robotframe{i}},\axis{z}{\robotframe{i}}\}$ and the frame of the payload is $\loadf$ with axes $\{\axis{x}{\loadf},\axis{y}{\loadf},\axis{z}{\loadf}\}$. Fig.\ref{frame_definition} illustrates aforementioned frames.
%\section{Overview}\label{sec:modeling}
The Payload Interactive Control Kit (PICK) is a high-level control pipeline that enables safe interactions between human operator and cable-suspended-payload via direct force contacts. PICK allows a human operator to directly interact with a payload suspended by multiple MAVs via force. The robot team will react to the external forces applied on the payload and move it to a desired location. Each MAV will also move away from human without affect payload's position. 

PICK employs a hierarchical control and estimation formulation starting from the payload external wrench estimator described in ~\ref{sec:Wrench_Estimator}, allowing 6D external wrench estimation on the rigid-body payload. These quantities are then sent to an admittance controller, which updates the desired payload position and velocity, as presented in Section ~\ref{sec:admittance_controller}. A lower-level payload controller based on our previous work \textcolor{red}{[ref]} then distributes desired thrust and moment to each robot based on cable geometry. The payload, suspended by varying numbers of MAVs, can be manipulated around by a human operator, and a safety controller, as discussed in ~\ref{sec:safety_controller}, is added to the control pipeline by exploiting the redundancy posted by having multiple MAVs in the form of null space to ensure a safe minimum distance between human operator and each of the flying MAVs without sacrificing payload position tracking.


A team of Micro Aerial Vehicles (MAVs) have
great potential in many commercial or health care settings
because of its flexible structure, robustness against disturbances,
and superior capability against each individual MAV. However,
human operators may find controlling a team more challenging
than an individual MAV. In this paper, we address this issue
with Payload Interactive Control Kit (PICK), a high level force-
based control pipeline designed to give human operator easy
and safe control over a team of payload-tranporting MAVs. The
key contributions are (a) a distributed, sensor-free, UKF-based
payload external wrench estimator that can be easily deployed
regardless of number of MAVs, (b) an 6D admittance controller
for the payload, and (c) an operator safety controller that
ensures a minimum safety distance between each MAV with the
operator by exploiting the redundancy post by using multiple
MAVs. Furthermore, we amended our previous work on Ro-
torTM (Simulator for Aerial Transportation and Manipulation)
with an external force module that allows testing of general
human-robot interaction within the simulation environment.
[The proposed scheme is validated through both simulation
and real-world experiments.]


%Particularly, aerial transportation offers a faster and more versatile solution compared to ground transportation in a congested urban environment. In addition, in post-disaster scenarios, a team of aerial robots can deliver supplies and establish communication in areas where GPS signal is intermittent or unavailable. To increase the payload capacity, one can either use a large aerial vehicle or utilize a team of MAVs that cooperatively transport a payload. Although the complexity of the system increases with the number of robots, a team of MAVs can potentially provide additional resilience to the task compared to a single MAV in case of vehicle failure. Furthermore,~\cite{Stolaroff2018} suggests that small scale drone-based delivery systems can potentially reduce greenhouse gas emissions and energy use in the freight sector. In this work, we investigate the control, state estimation, and trajectory tracking problems of distributed cooperative transportation of cable-suspended rigid body payloads with MAVs using a monocular camera and inertial sensor.

Specifically, the null space of ${\matP}$, $\mathcal{N}({\matP})$, which is the null mapping between the cable tension vectors and payload wrench, is the key to quantify such redundancy. Assume we find a possible tension vector $\nullspacev{}=\begin{bmatrix}\hdots & \nullspacev{\id} & \hdots\end{bmatrix}^{\top}$ and $\nullspacev{}$ is in $\mathcal{N}({\matP})$, where $\nullspacev{\id}=\begin{bmatrix}\nullspacevscalar{\id}^x & \nullspacevscalar{\id}^y & \nullspacevscalar{\id}^z\end{bmatrix}^{\top}$ is the null space tension vector for the $\id^{th}$ robot:

Effects similarly to gravity compensation on rigid link robots can be achieved given accurate estimation of external forces applied on the payload. A detailed presentation of the payload external wrench estimator is presented in Section~\ref{sec:Wrench_Estimator}.

The key contributions are (a) a distributed, sensor-free, UKF-based payload external wrench estimator that can be easily deployed regardless of number of MAVs, (b) an 6D admittance controller for the payload, and (c) an operator safety controller that ensures a minimum safety distance between each MAV with the operator by exploiting the redundancy post by using multiple MAVs. The proposed scheme is validated through both simulation and real-world experiments.

\begin{figure}[t]
    \centering
        \subfigure[Payload correction task asks the human operator to move the payload in from its current trajectory to prevent collision on an originally unknown obstacle.]{
         \includegraphics[width=\columnwidth]{figs/hardlimit_start2goal_nonzerok.png}
         \label{fig:avoid_obstacle_task}
         }
        \subfigure[Comparison between actual trajectory, desired trajectory, and admittance controller output. left: with optimization based safety controller. right: with gradient-based safety controller]{
         \label{fig:avoid_obstacle_task_plot}
         \includegraphics[width=\columnwidth]{figs/experiments/human_guided_avoid_obstacle_vertical.png}}
         \caption{}
\end{figure}


\makeatletter
\g@addto@macro\@maketitle{
\setcounter{figure}{0}
\centering
    \includegraphics[width=\linewidth]{figs/intro_4.0.jpg}
	\captionof{figure}{A Human operator collaborating with three quadrotors to transport a payload. On the Left: Quadrotors are expanding to keep safe distance from human without affecting payload position; On the Right: a payload is transported purely based on human operator's interactive force as command.\label{fig:Intro}}
	%\vspace{-3ex}
}
\makeatother

Although the system complexity increases with the number of robots, a team of MAVs possesses ability to manipulate large size and heavy payloads compared to a single MAV. In addition, they can potentially provide additional resilience to the task.

There are many possible application scenarios where we can apply autonomous transportation and manipulation with MAVs.

In fact, by considering MAVs equipped with ball joints~\cite{tagliabue2017icracollaborativetransportation}, magnets~\cite{LoiannoRAL2018} or gripper~\cite{Mellinger2013}, the robot team does not have the flexibility to create any safety distance between human operators. To physically cooperate with MAVs team with high-speed spinning propellers, it might create significant anxiety and pressure to the human operators, making them feeling unsafe.

%They generally add additional inertia to the system and may not be able to provide the sufficient maneuverability and flexibility to execute multiple tasks or preserve human operator safety .

%cons:additional inertia, reduced safety increased manipulation and transportation capabilities

%For instance, it is more challenging and sometimes infeasible to have non-cable attach mechanism to 1) transport or manipulate a payload, 2) to physically collaborating with a human operator, and 3) to concurrently ensure a safe operating distance among the robots and the human operator. 

%For example, several works can create safety distance between the agents using robot arms~\cite{thomas2014toward,afifi2022icraphysicalinteractionaerialmanipulator} or rigid links ~\cite{wang2018icra}, but this comes at the price of increased system inertia. %However, large safety distance comes at the cost of system inertia in these proposed designs. Cables, however, does not have this shortcoming. Based the above, cable-based solutions stand out uniquely among other attaching mechanisms for human-aerial-robot collaborative transportation and manipulation.


%The additional degrees of mobility between the robots and the load introduced by the cables, as well as their light-weight property can endow the system with the additional flexibility and safety. It allows simultaneous execution of multiple tasks, including cooperatively transport a payload, explore environments, change formation to avoid obstacle and maintain safety distance among the team and the human operator.

%First, we propose a scalable and distributed force-sensor-free payload external wrench estimator. Second, we formulate a 6D admittance controller for human-robot collaborative transportation and manipulation of a cable-suspended payload with a quadrotor team. Third, we augment the load controller with a module that can enhance the human safety by exploiting the additional degrees of mobility of the system introduced by using multiple agents. Specifically, compared to existing works, our controller considers the complete nonlinear dynamics of the quadrotor team carrying a tethered rigid-body payload, while offering the ability to preserve human or robot safety. Finally, a set of extensive real-world experiments validate the proposed approach. 

% to the authors' best knowledge, this is the first time a human operator can collaborate with a team of quadrotors to transport or manipulate a cable-suspended rigid-body payload meanwhile the quadrotor team keep safety distance with the human operator.

As mentioned above, the human operator's additional guidance or collaboration with the robot team can help the overall task. Human-robot interaction can be achieved in several complementary ways. The first approach is \textit{human-robot interaction through teleoperation}. In \cite{gengJGCD2020, gengImplementationDemonstrationCoordinated2019}, a state machine is designed for a human operator to command the entire quadrotor team to transition among hover, move, land, and take off. A similar approach is also proposed in~\cite{cano2022jirs}, where the authors propose a shared control structure such that the human operator can remotely send the payload's desired pose via a joystick. After obtaining the desired payload pose, the framework would generate desired position and velocity from the robot team to track based on an inverse kinematic controller in~\cite{sanalitro2020ralfullposecontrol}. In~\cite{pratik2020icra}, the human operator employs a remote controller to control the leader quadrotor. The remaining quadrotors in the team will follow the leader to transport the payload collaboratively. However, the "teleoperation approach" does not remove the system's dependency on the onboard controller and state estimation to maintain high precision tracking and may not provide a suitable human operator's interaction in certain tasks. 


In Section IV of the paper, we explain that the motion capture system is used to provide measurements for the Unscented Kalman Filter (UKF) that we have designed. The UKF utilizes motor speeds and a nonlinear dynamics model to predict the quadrotor states, including the tension force vector at the quadrotor, without the need for force sensors. In the updated manuscript, we present results demonstrating that the UKF-based estimation closely approximates the ground truth, even without the presence of force sensors. This showcases the effectiveness of our estimation approach in providing accurate estimates of the tension forces.

Additionally, we would like to clarify that in our previous works [12], we have developed an onboard estimation system that can estimate all the information collected by the motion capture system in this paper. We have validated this method by comparing the states from the onboard estimation system with those obtained from the motion capture system. Our previous research demonstrates that the onboard estimation system provides results close to the motion capture system, with cm-level errors. From our point of view, we can use our developed estimation method to replace the motion capture system to provide measurements to the UKF we designed in this paper. 

\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/experiments/impedance_1.png}
         \caption{$y=x$}
         \label{fig:y equals x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/experiments/impedance_2.png}
         \caption{$y=3\sin x$}
         \label{fig:three sin x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/experiments/impedance_3.png}
         \caption{$y=5/x$}
         \label{fig:five over x}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/experiments/impedance_4.png}
         \caption{$y=5/x$}
         \label{fig:five over x}
     \end{subfigure}
        \caption{Three simple graphs}
        \label{fig:three graphs}
\end{figure*}
\begin{table*}[t]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        &   Distributed & Scalable & Time Complexity\\
        \hline
      Quadrotor Controller&  Yes & Yes & $\mathcal{O}(1)$\\
      \hline
      Payload Trajectory Tracking Controller&  No & Yes & $\mathcal{O}(1)$\\
      \hline
      Gradient-Based Safety Controller&  Yes & Yes & $\mathcal{O}(1)$\\
      \hline
      Optimization-Based Safety Controller&   No & No & $\mathcal{O}(n^3)$\\
      \hline
      Payload Admittance Controller&  No & Yes & $O(1)$\\
      \hline
      Tension Distribution&  No & Yes & Exp: $\mathcal{O}(n)$ / Theory: $\mathcal{O}(1)$\\
      \hline
      Quadrotor Estimation&  Yes &  Yes & $\mathcal{O}(1)$\\
      \hline
      Payload Wrench Estimation&  No & Yes & $\mathcal{O}(n)$\\
      \hline
    \end{tabular}
    \caption{Scalability table (No Controller/State Est, can be used with new BD)}
    \label{tab:complexity}
\end{table*}
\begin{table*}[t]
\caption {Scalability table\label{tab:complexity}} 
\centering
%\newcolumntype{s}{}
\begin{tabularx}{\textwidth}{>{\hsize=1.5\hsize}X >{\hsize=0.58\hsize}X >{\hsize=0.58\hsize}X >{\hsize=0.5\hsize}X}
    \hline\hline
&Distributed & Scalable & Time Complexity\\\hline
\makecell{\cellcolor{mygreen}Human Interaction}&\makecell{\cellcolor{mygreen}}&\makecell{\cellcolor{mygreen}}&\makecell{\cellcolor{mygreen}}\\\hline
Quadrotor Estimation & Yes & Yes & $O(1)$\\
Payload Wrench Estimation & No & Yes & $O(n)$\\
Payload Admittance Controller & No & Yes & $O(1)$\\
\hline
\makecell{\cellcolor{myblue}Control}&\makecell{\cellcolor{myblue}}&\makecell{\cellcolor{myblue}}&\makecell{\cellcolor{myblue}}\\\hline
Quadrotor Controller& Yes & Yes & $O(1)$\\
Payload Trajectory Tracking Controller & No & Yes & $O(1)$\\
Gradient-Based Safety Controller & Yes & Yes & $O(1)$\\
Optimization-Based Safety Controller & No & No & $O(n^3)$\\
Tension Distribution & No & Yes & Experimentally $O(n)$ Theoretically $O(1)$\\\hline
\hline\hline
\end{tabularx}
\vspace{-10pt}
\end{table*}



Marked by its distributive design, our met enables onboard state estimation for each quadrotor, a feature that significantly enhances the system's scalability. As the size of the quadrotor swarm increases, there is no corresponding increase in computation cost per robot due to onboard processing. Moreover, the distributed design also minimizes potential interferences amongst the quadrotors, as estimation algorithms operate independently in parallel.

State estimation is performed fully onboard each quadrotor. The distributed nature of our method allows the entire system to be scaled easily. Since the estimation algorithm runs onboard, the computation cost per robot does not increase as the swarm gets large. The distributed design also reduces possible interference among robots as estimation algorithms are running independently in a parallel fashion. 

\begin{table}[t!]
  \centering
  \caption{Robot Types and Parameters.}\label{tab:robot_parameters}
%  \begin{tabularx}{\textwidth}{>{\hsize=0.225\hsize}X|>{\hsize=0.225\hsize}c|>{\hsize=0.225\hsize}c|>{\hsize=0.225\hsize}X}
\begin{tabularx}{\columnwidth} { 
   >{\raggedright\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X 
   >{\centering\arraybackslash}X 
   {\centering\arraybackslash}X}
%  \begin{tabular}{ | c m{5em} | m{5cm}| m{5cm} | m{5cm}| } 
    \hline\hline
    & Robot Arm\cite{afifi2023icuas} & Gripper~\cite{} & Magnet~\cite{LoiannoRAL2018} & Ball Joint~\cite{tagliabue2019ijrr} & Cable~\cite{guanrui2021ral} \\ 
    &\begin{minipage}{.1\columnwidth}
    %\centering
      \includegraphics[width=10mm, height=10mm]
      {figs/simulation/snapdragon.png}
    \end{minipage}
    &\begin{minipage}{.1\columnwidth}
    %\centering
      \includegraphics[width=10mm, height=10mm]
      {figs/simulation/snapdragon.png}
    \end{minipage}
    &\begin{minipage}{.1\columnwidth}
    %\centering
      \includegraphics[width=10mm, height=10mm]
      {figs/simulation/snapdragon.png}
    \end{minipage}
    &\begin{minipage}{.1\columnwidth}
    %\centering
      \includegraphics[width=10mm, height=10mm]
      {figs/simulation/hummingbird.png}
    \end{minipage}
    & \begin{minipage}{.1\columnwidth}
    %\centering
      \includegraphics[width=10mm, height=10mm]
      {figs/simulation/race.png}
    \end{minipage}
    \\\hline 
    Weight & 0.25 & 0.5 & 0.95 \\
Mechanical Design& 0.1075 & 0.17 & 0.10125 \\
Extra Actuation& 0.601$\times10^{-3}$ & 2.64$\times10^{-3}$ & 3.0$\times10^{-3}$ \\
Manipulability& 0.589$\times10^{-3}$ & 2.64$\times10^{-3}$ & 3.0$\times10^{-3}$ \\
    \hline\hline
  \end{tabularx}
  %\end{tabular}
\end{table}


\subsection{Potential of Using Onboard Sensing and Perception}
Throughout this paper, we employ a motion capture system for multiple purposes: 
\begin{enumerate}[label=\roman*)]
\item providing feedback on the payload states (pose and velocity) to the controller;
\item supplying measurement updates on the drone and cable states for the UKF on each drone, where the UKF utilizes motor speeds and a nonlinear dynamics model to predict drone states, including the tension force vector, without using force sensors; 
\item and providing the position of the human operator in the world.
\end{enumerate}


We argue that the state estimation can be replaced with onboard sensing due to several reasons. As discussed in~\cite{guanrui2021ral}, 
we designed an Extended Kalman Filter (EKF) to predict the cable direction and velocity through the nonlinear dynamics model using the IMU data and motor speeds from the Electronic Speed Controller (ESC). By employing a black-and-white circular tag attached at each cable's end and applying the computer vision algorithm from~\cite{whycon_jint}, we can obtain the measurement of the attach point position with respect to the robot frame at $30$ Hz camera rate. Given the assumption that the cable remains taut, we can leverage the geometry constraints and the robot's orientation estimated by the onboard Visual-Inertial Odometry (VIO) algorithm to measure the cable's direction with respect to the world frame. The measured cable direction above serves as a measurement update to the EKF, ensuring our estimate remains accurate and responsive. With the proposed EKF estimator, we can obtain the cable direction $\cablevec{}$ and velocity $\cabledotvec{}$ up to 250 Hz. 

Furthermore, we can also leverage the quadrotor position estimated from the onboard VIO and the estimated cable direction from above, under the taut cable assumption, to infer the attach point position in the world frame. By sharing the positions of all attach points among the robots, they can collectively estimate the payload state, pose, and velocity, which can then be used as feedback for the payload controller.

In~\cite{guanrui2021ral}, we validate the vision-based state estimation method by comparing the states from the onboard estimation system with those obtained from the motion capture system. The results indicate that the onboard estimation system provides comparable outcomes to the motion capture system, with only cm-level errors. Hence, this technique can potentially provide all necessary measurement updates for the UKF developed in this paper. 
Finally, theoretically, we can also obtain the position of the human using onboard cameras by leveraging state-of-the-art human pose estimators~\cite{rennips2015fasterrcnh}.

To quantitatively support our analysis, we conducted multiple iterations of the same experiments and recorded the distances between the robots and the human operator. The distribution of these distance measurements is illustrated in Figs.~\ref{fig:optimization-analysis} and \ref{fig:gradient-analysis}, with corresponding mean and standard deviation values summarized in Table~\ref{tab:distance_summary}.

As shown in Figs.~\ref{fig:optimization-analysis} and \ref{fig:gradient-analysis}, both the optimization-based and gradient-based methods effectively maintain a consistent distance between the robots and the human operator. This observation is further validated by the statistical data presented in Table~\ref{tab:distance_summary}. Notably, the optimization-based method distinguishes itself from the gradient-based method as it enforces inter-robot distance constraints. This is evident in the top plot of Fig.~\ref{fig:transportation_distance_opt}, where all three drones maintain a minimum separation of $0.75\si{m}$, as specified by the constraint.

To provide additional context, Figs.~\ref{fig:transportation_distance_grad} and \ref{fig:transportation_distance_opt} depict sample trajectories of the distances between each robot and the human operator, as well as the inter-robot distances, throughout the duration of a single experiment. Initially, the human operator starts approximately $2$ to $3\si{m}$ away from the robot team. As the operator approaches, the distances between the human and robots 1 and 3 (represented by blue and green) decrease to around $0.75~\si{m}$. At this point, the human-aware force distribution becomes active, stabilizing the human-robot distances around the $0.75~\si{m}$ threshold.
